Improving Masked Autoencoders by Learning Where to Mask

Masked image modeling is a promising self-supervised learning method for visual data. It is typically built upon image patches with random masks, which largely ignores the variation of information density between them. The question is: Is there a better masking strategy than random sampling and how can we learn it? We empirically study this problem and initially find that introducing object-centric priors in mask sampling can significantly improve the learned representations. Inspired by this observation, we present AutoMAE, a fully differentiable framework that uses Gumbel-Softmax to interlink an adversarially-trained mask generator and a mask-guided image modeling process. In this way, our approach can adaptively find patches with higher information density for different images, and further strike a balance between the information gain obtained from image reconstruction and its practical training difficulty. In our experiments, AutoMAE is shown to provide effective pretraining models on standard self-supervised benchmarks and downstream tasks.

==> text/supp_backup.tex <==
\section{Model Analyses}

We conduct model analyses in the linear probing setup by pretraining the models on smaller subsets of ImageNet-1K.
%
% \paragraph{Setup.} We randomly sample $100{,}000$ images from the ImageNet-1K dataset. More specifically, we randomly selected $100$ images for every class in those images with bounding box annotations. Based on a balanced dataset with bounding box ground truth, we conduct experiments in Fig.~\ref{fig:preliminary} and take it as a reference.
% \vspace{-2mm}
%
Specifically, we randomly sample $10\% \sim 30\%$ images and perform the pretraining for $400$ epochs. For linear probing, we finetune the model for $90$ epochs and evaluate it on the \textbf{full} ImageNet-1K validation set. 
% We use a $10\%$ subset in the experiment shown in Table~\ref{tab:ablations-supplementary}.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}


% \vspace{-2mm}
% \paragraph{Different pretrained ViT in mask generator.} We replace original MAE-800 ViT-encoder with the MAE baseline ($22.89$) pretrained on the subset with $400$ epochs to train another AutoMAE, term as ``AutoMAE (MAE-400-small)''. It obtains significantly higher ($+2.89$) than its baseline MAE. It also outperforms the best raising probability model in Fig.~\ref{fig:preliminary}. It shows that the method is effective even without a pretrained model on a big dataset,
% \vspace{-2mm}

\paragraph{Mask generator with a pretrained ViT.} 
In Table \ref{tab:ablations}, we compare the use of different self-supervised warmup methods (MAE-800 vs. MAE-400-Small) for the ViT-Base feature extractor in the mask generator. 
%
The latter one is \emph{pretrained on the $30\%$ subset for $400$ epochs}. 
%
It achieves a comparable Top-1 accuracy ($53.57\%$) with the one with the MAE-800 backbone ($53.58\%$), which is significantly higher ($+2.89$) than its baseline MAE ($50.50\%$) and the best MAE model with ground-truth bounding box guidance (as described in Section 2.2 of the paper). %~\ref{sec:preliminary_observation}).
%
These results indicate that the main improvement in the performance of AutoMAE comes from the differentiable mask sampling method, as the mask generator is effective even with a weak feature extractor.


\begin{table}[h]
\begin{center}
\begin{tabular}{|L{3cm}|L{3cm}|C{2cm}|}
\hline
Model  & Warmup in $G$  & Acc-1(\%)  \\ \hline
MAE~\cite{he2022masked}   & N/A & 50.50 \\
| w/ bounding box & N/A & 52.52 \\
\hline
AutoMAE & MAE-400-Small & 53.57 \\
AutoMAE  & MAE-800  & 53.58 \\
| Two-Stage & MAE-800 & 52.57 \\
| $G:$ MAE-Max   & MAE-800 & 50.85 \\
AutoMAE & DINO-B     & 53.20 \\
| $G:$ DINO-Max  & DINO-B & 51.52 \\ \hline
\end{tabular}
\end{center}
\vspace{-5pt}
\caption{Linear probing accuracy of models pretrained on a $30\%$ subset of ImageNet-1K for $400$ epochs. All models are on the full validation set of ImageNet-1K. We use different ViT backbones with frozen parameters in the mask generator.}
\label{tab:ablations}
% \vspace{5pt}
\end{table}

\begin{table}[t]
% \vspace{-10pt}
\begin{center}
\begin{tabular}{|L{3cm}|L{3cm}|C{2cm}|}
\hline
Model & Warmup in $G$    & Acc-1(\%)  \\ \hline
% MAE~\cite{he2022masked}  & N/A     & 23.07 $\pm$ 0.13\\ 
% \hline
% AutoMAE & MAE-800   &26.84 $\pm$ 0.18 \\
% AutoMAE & iBOT-B \cite{zhou2021ibot}  & 26.47 $\pm$ 0.17 \\ 
MAE~\cite{he2022masked}  & N/A     & 23.07 \\ 
AutoMAE & MAE-800   &\textbf{26.84}  \\
% AutoMAE & iBOT-B \cite{zhou2021ibot}  & \underline{26.47}  \\ 
% AutoMAE & DINO-S \cite{caron2021emerging}    & 26.20 \\
\hline
AutoMAE & From-Scratch    & \underline{26.00} \\ 
| w/ EMA $m=0.9$ & From-Scratch& 25.92 \\ 
| w/ EMA $m=0.99$ & From-Scratch& 25.45 \\ \hline
\end{tabular}
\end{center}
\vspace{-5pt}
\caption{Linear probing of models pretrained on $10\%$ ImageNet for $400$ epochs. AutoMAE outperforms the original MAE pertaining even with a randomly initialized mask generator.
% The first $3$ three models are pretrained for $3$ times.
}
\label{tab:ablations-supplementary}
% \vspace{-10pt}
\end{table}

\begin{table}[t!]
\begin{center}
\begin{tabular}{|L{3cm}|C{1cm}|C{1cm}|C{1cm}|}
\hline
$\beta$             & 0.2   & 0.5   & 1.0 \\ \hline
Linear probing     & 52.04 & 53.58 &  53.43  \\ \hline
\end{tabular}
\end{center}
\vspace{-5pt}
\caption{Linear probing accuracy with different margin values.}
\label{tab:beta_search}
% \vspace{-20pt}
\end{table}

% \vspace{-2mm}
% \paragraph{Two-stage training.} SemMAE \cite{li2022semmae} trains the mask generator first and then trains the target model. By contrast, our model train the mask generator and the MAE model together. In this experiment, we first pre-train a normal AutoMAE to get its best accuracy and then use the fixed weight of the two-layer convolution generator along with MAE-800 to generate masks. As shown by the ``Two-stage'' results in Table \ref{tab:ablations}, it is still higher than MAE but significantly worse than AutoMAE(MAE-800). ($25.87$ vs $27.04$)
% \vspace{-2mm}

\paragraph{Mask generator without a pretrained ViT.} 
In most of the experiments, the mask generator of AutoMAE relies on a pretrained ViT. We here consider removing such a requirement by using a train-from-scratch ViT backbone. The simplest way is to \textbf{reuse} the same ViT model for both mask generation and mask reconstruction.
%
As shown in Table~\ref{tab:ablations-supplementary}, this model (``From-Scratch'') remarkably outperforms the vanilla MAE model ($26.00\%$ vs $23.07\%$), both pretrained on the $10\%$ ImageNet subset.
%
It suggests that AutoMAE is effective even without any pretrained models.
%
We further perform the exponential moving average (EMA) to synchronize the ViT used for mask generation ($k$) and the one used for image reconstruction ($q$). We have $\theta_k = m \times \theta_k + (1-m) \times \theta_q$. 
%
Results are shown in Table~\ref{tab:ablations-supplementary}.
 

\paragraph{On joint training.} 
We conduct an ablation study of AutoMAE by separating it into two independent learning processes, i.e., mask generation and mask-guided image modeling.
%
In Table \ref{tab:ablations}, the ``Two-stage'' model outperforms MAE ($52.57\%$ vs $50.50\%$) but underperforms the joint training version ($53.58\%$), which validates the effectiveness of joint training in AutoMAE.
%
In Table 1 of the paper (\textit{full-set pretraining}), we compare AutoMAE with SemMAE, a two-stage pretraining pipeline with an independent mask learning stage. It further supports the superiority of joint training over two-stage training ($66.7\%$ vs. $65.0\%$). 


% In addition, considering that SemMAE uses a two-stage pretraining pipeline with an independent mask learning stage, we compare it with AutoMAE to further evaluate the effect of joint training.
%As shown in Table \ref{tab:linear-probing} (\textit{full-set pretraining}), 

\paragraph{On adversarial mask generation.} As DINO \cite{caron2021emerging} suggests that the last self-attention layer in ViT blocks can provide meaningful masks, we remove the adversarial training loss and replace the two-layer CNN in the mask generator (after the feature extractor) with a simple $\mathrm{maximum}$ operator over the channel axis. 
%
From Table \ref{tab:ablations}, although these models (``MAE-Max \& DINO-Max'') still outperform the original MAE, they obtain lower accuracy than corresponding AutoMAE models with MAE-800 and DINO-B.
%
It indicates that the mask generator does learn a better masking function than simply taking the maximum attention values.

\paragraph{Sensitivity analysis on the margin value $\beta$.} Previously in Fig.~\ref{fig:preliminary}, we show how the margin value of the masking probability $\beta$ affects the linear probing performance with bounding box guidance. Here, as shown in Table \ref{tab:beta_search}, we conduct a grid search over $\beta=\{0.2, 0.5, 1.0\}$ on the ImageNet subset and find that $\beta=0.5$ performs best. 


\section{Implementation Details}
\label{pre-train-section}


\paragraph{Model architecture.} 
\vspace{-2mm}
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.7\linewidth]{fig/discriminator.pdf}
\caption{The architecture of the mask discriminator.}
\label{fig:discriminator}
\end{center}
\vspace{-18pt}
\end{figure}
% We employ the official implementation of MAE~\cite{he2022masked} as our self-supervised learning method and conduct model pretraining on the ImageNet-1K dataset~\cite{DBLP:conf/cvpr/DengDSLL009}.
In adversarial training, we use a three-layer CNN as the discriminator. The first two convolutional layers have a $4\times4$ kernel size, a stride of $2$, and a zero-padding length of $1$. They are followed by a Spectral Normalization~\cite{DBLP:journals/corr/YoshidaM17} layer and a LeakyReLU activation. The LeakyReLU has a negative slope of $0.2$. The last convolutional layer has a filter size of $3\times3$ and is also followed by a spectral normalization layer. As shown in Fig.~\ref{fig:discriminator}, the spatial size of feature maps is $14\rightarrow 7\rightarrow 3 \rightarrow 1$ and the number of channels is $1\rightarrow 16\rightarrow 32\rightarrow 1$.

 % As shown in Fig.~\ref{fig:discriminator}, the spatial size of feature maps is $14\rightarrow 7\rightarrow 3 \rightarrow 1$ and the number of channels is $1\rightarrow 16\rightarrow 32\rightarrow 1$.

% \vspace{-4mm}
\paragraph{Training details.} We adopt the AdamW optimizer \cite{DBLP:conf/iclr/LoshchilovH19} for pretraining the MAE model and the mask generator in our AutoMAE. Following previous work~\cite{he2022masked}, the base learning rate is set to $1.5\times 10^{-4}$, the momentum is configured as $\beta_1 = 0.9, \beta_2 = 0.95$, and the batch size is $4{,}096$. We use the linear learning rate schedule: \textit{lr} = \textit{base\_lr} $\times$ \textit{batchsize} $/ 256$. The weight decay is $0.05$. The learning rate is scheduled by cosine decay with a warm-up phase of $40$ epochs and the total number of pretraining epochs is set to $800$. We use random resized cropping and random horizontal flipping for data augmentation. 
%
For the discriminator, we use the Adam optimizer without the weight decay. Other hyper-parameters stay the same. The mask generator uses a margin of $\alpha = 0.5$ to highlight the randomly sampled foreground area, and the loss weight $\lambda$ is set to $0.2$ to balance generator loss with reconstruction loss.  

\paragraph{Hyperparameters tuning.}
In Eq.(4) and Eq.(6), we set $\alpha = \beta$ as they have similar effects. In Eq.(5), the values of $a,b,c$ are directly taken from LSGAN~\cite{DBLP:conf/iccv/MaoLXLWS17}. We only tune $\beta$ and the loss weight $\lambda$ on the ImageNet subset ($30\%$) and reuse the obtained values in other datasets/setups.


\paragraph{Training cost.} We use a patch size of $16\times 16$ for all experiments. It takes $26$ hours to pretrain an AutoMAE model on $30\%$ of ImageNet with $8$ NVIDIA RTX 3080Ti cards for $400$ epochs, and $7$ days to pretrain an AutoMAE model on the full ImageNet dataset with $8$ NVIDIA A100 cards for $800$ epochs. Admittedly, MAEs commonly benefit from a smaller $8\times8$ patch size. However, we cannot afford its training cost, \textit{e.g.}, it takes about $4$ weeks for $800$ epochs on the full ImageNet-1K. We want this paper to focus more on the proposed training scheme than on hyper-parameter tuning. Therefore, we follow the standard $16\times16$ setup~\cite{he2020momentum,zhou2021ibot}, which does not affect the main conclusions when compared to SemMAE.
%
As shown in Table~\ref{tab:compare}, AutoMAE has comparable time cost to recent advances in self-supervised pre-training \cite{10.1007/978-3-031-20056-4_18,li2022semmae} based on the same hardware ($8\times$A100 GPUs) for $800$ epochs. The full model has a similar number of FLOPs to existing work.

\section{Visualization}
\label{sec:3}

In Figure 4 in our paper, we show that the mask generator can perceive meaningful areas in examples from ImageNet-9~\cite{xiao2021noise}. In this section, we will explain the details and show more samples from ImageNet-1K~\cite{DBLP:conf/cvpr/DengDSLL009} during the pretraining process of AutoMAE.

After passing the ViT attention feature map to the two-layer CNN generator, the mask is obtained by applying $\log(\mathrm{softmax}(\cdot))$ and Gumbel softmax. Due to the randomness of Gumbel, we take the output of $\log(\mathrm{softmax}(\cdot))$ and highlight those tokens with the top $25\%$ probabilities. They are visualized in Figures~\ref{fig:masked1}-\ref{fig:masked3} as white patches. 

Figures~\ref{fig:masked1}-\ref{fig:masked3} indicate that the mask generator can learn the information of foreground objects. We can see that at the beginning of training, the mask has no specific patterns. After a certain period of training, it becomes focused on the foreground object. It can even follow the shape of discrete parts (see showcases 15 and 16). It shows that the mask tends to fit the shape of the foreground object best at the early stage (see showcases 3, 5-11). For complex scenes in Fig.~\ref{fig:masked3}, it still generates meaningful masks around at least one foreground object. Although the generated mask is gradually changed during the pretraining process, it is mainly focused on the area around the foreground, which indicates that it will have a high probability to be dropped in AutoMAE. It demonstrates that our model can generate semantic masks to improve the self-supervised learning process of the original MAE.

\begin{table}[t]
\begin{center}
\begin{tabular}{|l|c|c|C{3.5cm}|c|}
\hline
Method & Time (@800 epochs) & FLOPs & Hyper-parameters to tune & Better results   \\
\hline
% \hline
SemMAE~\cite{li2022semmae} & 6 days & Unknown & Partitions, Blur kernel,  $\gamma$, Patch size, $\lambda$ & 1/7 setups\\ 
\hline
AttMask \cite{10.1007/978-3-031-20056-4_18} & $\textgreater$ 8 days & 37.03G & \#Attn layers, $p$, $r$, $s$, $\lambda$ (see 
\cite{10.1007/978-3-031-20056-4_18} for details) & --\\ 
\hline
AutoMAE (ours)  & 7 days & 35.72G & $\alpha=\beta$, $\lambda$ & 6/7 setups\\ 
\hline %$\mathcal G$ (xxM), $\mathcal D$ (xxM), $\mathcal{B}$ (xxM)
\end{tabular}
\end{center}

\caption{
AutoMAE performs better \textbf{in $6/7$ setups}: Linear probing, $30\%$ finetuning, $100\% \& 50\%$ fine-grained classification, detection, and segmentation. It is worth noting that: (1) The mask generators in SemMAE and AutoMAE are both based on the pretrained ViT encoder; (2) AutoMAE has fewer hyperparameters to tune than SemMAE and AttMask.
}
\vspace{-20pt}
\label{tab:compare}
\end{table}


\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{fig/masked-images-1.pdf}
    \caption{Masked patches by AutoMAE during the pretraining for $800$ epochs. White patches are the output of $\log(\mathrm{softmax}(\cdot))$ with the top $25\%$ probabilities.}
    \label{fig:masked1}
\end{figure*}

\begin{figure*}[ht]
    \vspace{15mm}
    \begin{center}
        \includegraphics[width=\textwidth]{fig/masked-images-2.pdf}
        \caption{Masked patches by AutoMAE during the pretraining for 800 epochs. White patches are the output of $\log(\mathrm{softmax}(\cdot))$ with the top $25\%$ probabilities.}
    \label{fig:masked2}
    \end{center}
    \vspace{15mm}
\end{figure*}

\begin{figure*}[ht]
    \vspace{15mm}
    \begin{center}
        \includegraphics[width=\textwidth]{fig/masked-images-3.pdf}
    \caption{Masked patches by AutoMAE during the pretraining for 800 epochs. White patches are the output of $\log(\mathrm{softmax}(\cdot))$ with the top $25\%$ probabilities.}
    \label{fig:masked3}
    \end{center}
    \vspace{15mm}
\end{figure*}


% As shown in Table~\ref{tab:compare}, AutoMAE has comparable time cost to recent advances in self-supervised pre-training based on the same hardware ($8\times$A100 GPUs). The full model has a similar number of parameters and FLOPs to existing work.

% \begin{table*}[b]
% \vspace{-10pt}
% \footnotesize
%     \centering
% \begin{tabular}{|l|ccccc|}
% \hline
% Method & Time (@$800$ epochs) & \# Params in total & FLOPs & Hyper-parameters to tune & Better results   \\
% \hline
% % \hline
% SemMAE [23] & 6 days & Unknown & Unknown & Partitions, Blur kernel,  $\gamma$, Patch size, $\lambda$ & 1/7 setups\\ 
% \hline
% AttMask [21] & $\textgreater$ 8 days & 188.10M & 37.03G & \#Attn layers, $p$, $r$, $s$, $\lambda$ (see [21] for details) & --\\ 
% \hline
% AutoMAE (ours)  & 7 days & 198.08M & 35.72G & $\alpha=\beta$, $\lambda$ & 6/7 setups\\ 
% \hline %$\mathcal G$ (xxM), $\mathcal D$ (xxM), $\mathcal{B}$ (xxM)
% \end{tabular}
%     \caption{Further comparisons. The mask generators in SemMAE and AutoMAE are both based on the pre-trained ViT encoder, while AutoMAE performs better \textbf{in $6/7$ setups}: Linear probing, $30\%$ fine-tuning, $100\% \& 50\%$ fine-grained cls, detection, and segmentation.
% 	}
% 	\label{tab:compare}
% \end{table*}

% Notably, the mask generator and discriminator are only used in the pre-training phase. The ViT model used in linear probing and fine-tuning has the same network architecture as that in the original MAE paper. Therefore, we adopt the implementation details, including data augmentation and regularization strategies, from the official MAE Vit-Base. 

